ChildBot: Multi-Robot Perception and Interaction with Children

In this paper we present an integrated robotic system capable of participating in and performing a wide range of educational and entertainment tasks, in collaboration with one or more children. The system, called ChildBot, features multimodal perception modules and multiple robotic agents that monitor the interaction environment, and can robustly coordinate complex Child-Robot Interaction use-cases. In order to validate the effectiveness of the system and its integrated modules, we have conducted multiple experiments with a total of 52 children. Our results show improved perception capabilities in comparison to our earlier works that ChildBot was based on. In addition, we have conducted a preliminary user experience study, employing some educational/entertainment tasks, that yields encouraging results regarding the technical validity of our system and initial insights on the user experience with it.

==> action_res.tex <==
%
In order to verify the appropriateness of the proposed action and gesture recognition system in more challenging tasks, we evaluate the pantomime actions described previously. These actions are more complex than gestures since children perform them in many different ways. 
Table~\ref{tab:pres} presents the average accuracy results (\%) for the 12 gestures as well as the background model. Despite the difficulty of the task, the system performs quite well with fusion around $74\%$ for a 13 classes problem. 

For the further evaluation of  the action recognition system, as in the gesture recognition task,
we have trained a separate model for each Kinect sensor using as training sets: a) the children's gesture data, b) the adults' gesture data, and c) both. Testing was carried out for both children and adult data separately, using leave-one-out cross-validation. Table ~\ref{tab:pres2} presents the average accuracy (Acc.) results (\%) for the 12 pantomime actions and the background model, for every combination of training and test sets.
Results indicate that fusion of the three Kinect sensors improves significantly the performance compared to the best single sensor result. Also, when training and test data come from the same age group, the recognition accuracy is high.
Using the mixed training set deteriorates slightly the performance on both adults and children action recognition.

\begin{comment}
\begin{table*}[!tb]
\renewcommand{\arraystretch}{1.2}
\centering
\scriptsize
\begin{tabular}{|l|c|c|c|c|c|c|c|c||c|c|c|c|c|c|} \cline{2-15}
\multicolumn{1}{c|}{} & \multicolumn{14}{c|}{Development Data} \\ \cline{2-15}
           \multicolumn{1}{c|}{}  & \multicolumn{8}{c||}{Single Camera} & \multicolumn{6}{c|}{Fusion}\\\hline
Features      &  \multicolumn{2}{c|}{Kinect \#$1$}   & \multicolumn{2}{c|}{Kinect \#$2$}   & \multicolumn{2}{c|}{Kinect \#$3$}  & \multicolumn{2}{c||}{Kinect \#$4$}  & \multicolumn{2}{c|}{Features} & \multicolumn{2}{c|}{Encodings} & \multicolumn{2}{c|}{Scores} \\ \cline{2-15}
 & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD \\ \hline
 
HOF  & 68.31 & 69.85 & 56.31 & 63.08 & 48.62 & 50.46 & 53.85 & 63.69 & 66.77 & 67.08 & 68.00 & 69.23 & 68.62 & 75.50\\ 
MBH  &  70.77 & 72.92 & 60.92 & 68.62 & 61.85 & 60.00 & 55.22 & 72.92 & 76.00 & 76.69 & 76.92 & 76.92 & 74.46 & 76.50\\ 
Traj.+HOG+HOF+MBH & 73.85 & 74.15 & 63.38 & 69.23 & 60.00 & 58.46 & 61.45 & 76.31 & 75.08 & 76.92 & 77.23 & 77.85 & 75.08 & 79.00\\\hline 
\multicolumn{1}{c|}{} & \multicolumn{14}{c|}{Experimental Data} \\ \cline{2-15}
\multicolumn{1}{c|}{}  & \multicolumn{8}{c||}{Single Camera} & \multicolumn{6}{c|}{Fusion}\\\hline
Features      &  \multicolumn{2}{c|}{Kinect \#$1$}   & \multicolumn{2}{c|}{Kinect \#$2$}   & \multicolumn{2}{c|}{Kinect \#$3$}  & \multicolumn{2}{c||}{Kinect \#$4$}  & \multicolumn{2}{c|}{Features} & \multicolumn{2}{c|}{Encodings} & \multicolumn{2}{c|}{Scores} \\ \cline{2-15}
 & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD & BoW & VLAD \\ \hline
HOF  & 46.34 & 51.00 & 46.19 & 51.78 & 25.50 & 26.13 & 47.70 & 44.67 & 63.08 & 61.02 & 49.87 & 56.17 & 52.59 & 57.99\\
MBH  & 61.42 & 56.86 & 46.28 & 45.82 & 31.59 & 29.44 & 45.57 & 56.11 &  70.25 & 67.97 & 57.70 & 59.04 & 62.18 & 62.49\\
Traj.+HOG+HOF+MBH  & 52.59 & 59.16 & 46.74 & 51.51 & 36.62 & 38.22 & 48.16 & 55.11 & 63.52 & 69.37 & 60.75 & 61.55 & 55.00 & 64.90\\ \hline
\end{tabular}
\caption{Average classification accuracy (\%) for the employed 13 pantomimes performed by 28 children. Results for the five different features for both single and multi-stream cases.}
\label{tab:gres}
\end{table*}
\end{comment}


\begin{comment}
\begin{table}[!tb]
\centering
\begin{tabular}{|l|l|c|c|c|} \cline{3-5}
 \multicolumn{1}{c}{}  & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Action Recognition} \\ \cline{3-5}
\multicolumn{1}{c}{}  & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Training scheme} \\ \cline{1-5}
\multicolumn{2}{|c|}{Test}   & \multicolumn{1}{c|}{Adults}   &  \multicolumn{1}{c|}{Children}  & \multicolumn{1}{c|}{Mixed}   \\ \cline{1-5}
 \multirow{2}{*}{Adults} 
 & Avg & $78.39$ & $63.00$ & $78.39$ \\  
 & Fuse & $\textbf{87.36}$ & $72.53$ & $86.26$ \\  \cline{1-5}
\multirow{2}{*}{Children} 
 & Avg & $46.55$ & $65.74$  & $65.88$  \\ 
 & Fuse & $56.51$ & $\textbf{74.46}$  & $74.26$  \\ \hline
\end{tabular}
\caption{Evaluation of the action recognition modules.}
\label{tab:pres2}
\end{table}
\end{comment}

